Symplectically Integrated Symbolic Regression of Hamiltonian Dynamical Systems

Here we present Symplectically Integrated Symbolic Regression (SISR), a novel technique for learning physical governing equations from data. SISR employs a deep symbolic regression approach, using a multi-layer LSTM-RNN with mutation to probabilistically sample Hamiltonian symbolic expressions. Using symplectic neural networks, we develop a model-agnostic approach for extracting meaningful physical priors from the data that can be imposed on-the-fly into the RNN output, limiting its search space. Hamiltonians generated by the RNN are optimized and assessed using a fourth-order symplectic integration scheme; prediction performance is used to train the LSTM-RNN to generate increasingly better functions via a risk-seeking policy gradients approach. Employing these techniques, we extract correct governing equations from oscillator, pendulum, two-body, and three-body gravitational systems with noisy and extremely small datasets.

==> notes.tex <==
-----------------------------
Intro
-----------------------------


-----------------------------
Theory
-----------------------------

My main comment is about the structure and the novelty. It will be good to have an overview figure of the system and let each sub-section to correspond to one part of the system in the figure. Each sub-section should highlight its main contribution at the beginning of the first paragraph (what's new and what's the challenge addressed). Also, we need to list these contributions in the introduction as well (the second last paragraph).



- Figure 1: The title could be changed to system overview or network architecture. Also, should we move Figure 1 to Section 3.3 after you introduce SISR? Also, I am not sure if Fig 1 is a good overview picture (I didn't see the RNN component at least). If it is not, do we need an overview picture in Section 3.3? 

Then we have three figures in total: Fig 1 for the idea, Fig 2 for the system overview, and Fig 3 for the training loop.

- 3.3.5 Can be merged to the Experiment (e.g., after 4.5) and rename it as Comparison to Existing Approaches. Maybe. Not sure. It might be good to put it here too.

- One thing we need to say explicitly is the novelty of the approach. It will be good to say this at the beginning of each section when you start to introduce a technical contribution. We can say it explicitly like "We propose a novel RNN component to ... "

-----------------------------
Experiment
-----------------------------
This section looks good to me. My only comment is to emphasize that we use small training data sets for all examples (highlight this at the beginning of Section 4 and in each sub-section).


-----------------------------
Conclusion
-----------------------------
A few sentences for future work?

######################
# Post-Revision Notes
######################
